Towards Understanding Extrapolation: a Causal Lens

Canonical work handling distribution shifts typically necessitates an entire target distribution that lands inside the training distribution. However, practical scenarios often involve only a handful of target samples, potentially lying outside the training support, which requires the capability of extrapolation. In this work, we aim to provide a theoretical understanding of when extrapolation is possible and offer principled methods to achieve it without requiring an on-support target distribution. To this end, we formulate the extrapolation problem with a latent-variable model that embodies the minimal change principle in causal mechanisms. Under this formulation, we cast the extrapolation problem into a latent-variable identification problem. We provide realistic conditions on shift properties and the estimation objectives that lead to identification even when only one off-support target sample is available, tackling the most challenging scenarios. Our theory reveals the intricate interplay between the underlying manifold's smoothness and the shift properties. We showcase how our theoretical results inform the design of practical adaptation algorithms. Through experiments on both synthetic and real-world data, we validate our theoretical findings and their practical implications.

==> sections/methods.tex <==


\section{Algorithms}


\subsection{Implementation} \label{subsec:implementation}

Given these two conditions, we present our model diagram in Figure~\ref{fig:vae_model} and the objective function in Equation~\ref{eq:objective}.

\begin{figure}[h]
    \centering
    \includegraphics[width=.66\textwidth]{figures/vae.png}
    \caption{\textbf{The model diagram and loss functions.} }
    \label{fig:vae_model}
\end{figure}

Formally, we optimize the following objectives:
\begin{align} \label{eq:objective}
\begin{split}
    &\cL(\enc, \dec, \cls): = \\
    &\EE{
        \xx
    }{
    \EE{
        \cc \sim q ( \cc | \xx ), \ss \sim q ( \ss | \xx ) 
    }{
        \log \left( p( \xx | \cc, \ss ) \right)
    } \qquad \text{(reconstruction)}} \\
    % & + \lambda_{\text{recons\_tgt}} \cdot \EE{
    %         \xx_{\text{tgt}}
    %     }{
    %     \EE{
    %         \cc_{\text{tgt}} \sim q ( \cc | \xx_{\text{tgt}} ), \ss_{\text{tgt}} \sim q ( \ss | \xx_{\text{tgt}} ) 
    %     }{
    %         \log \left( p( \xx_{\text{tgt}} | \cc_{\text{tgt}}, \ss_{\text{tgt}} ) \right)
    % } \qquad \text{(target reconstruction)}} \\
    & + \lambda_{\text{KL}} \cdot \left( D ( q ( \cc | \xx_{\text{src}} ) || p ( \cc ) ) \right)
    \qquad \text{(KL regularization)} \\
    & - \lambda_{\text{nat}} \cdot \EE{
            \xx_{\text{tgt}}
        }{
        \EE{
            \cc_{\text{tgt}} \sim q ( \cc | \xx_{\text{tgt}} )
        }{
            \log \left( p( \cc_{\text{tgt}}) \right)
    } \qquad \text{(naturalness)}} \\
    & + \lambda_{\text{ cls }} \cdot \EEb{\xx_{\text{src}}, \yy_{\text{src}}}{ \EEb{ \cc_{\text{src}} \sim q(\cc | \xx_{\text{src}}) }{\text{CrossEntropy}(\yy_{\text{src}}, \cls(\cc_{\text{src}})} } \qquad \text{(classification)} \\
    & + \lambda_{\text{anti-nat}} \cdot \left( { \color{red} D ( q ( \ss | \xx_{\text{src}} ) || p ( \ss) ) + \EE{
            \xx_{\text{tgt}}
        }{
        \EE{
            \ss_{\text{tgt}} \sim q ( \ss | \xx_{\text{tgt}} )
        }{
            p( \ss_{\text{tgt}})
    } } } \right) \qquad \text{(anti-naturalness)}. 
    % & + \lambda_{\text{dim}} \cdot \EEb{ \xx }{ \EEb{ \ss \sim q ( \ss | \xx )}{ \norm{ \ss }_{0} } }  \qquad \text{(dimension control)} .
\end{split}
\end{align}





\subsection{Source-free Approximation}

In practice, the source-distribution samples are often unavailable.
We adopt approximations in our algorithm to combat this issue.
In practice, the source samples are often unavailable at the test time. Much work has been devoted to source-free test-time adaptation.
\begin{itemize}
    \item We can view minimizing entropy $ \sum_{ i } - \hat{P}( \hat{ \yy } = \yy_{i} ) \log( \hat{P}( \hat{ \yy } = \yy_{i} ) ) $ as an surrogate of maximizing $ p( \hat{\zz} ) $ -- the entropy is minimized when $ \hat{\zz} $ attains the highest the density value.
    \item We can add a soft mask with sparsity regularization to automatically select $\hat{\cc}$ for the entropy estimation (Figure~\ref{fig:entropy_model}).
\end{itemize}


\begin{figure}[h]
    \centering
    \includegraphics[width=.66\textwidth]{figures/entropy.png}
    \caption{\textbf{Our method with entropy minimization.} }
    \label{fig:entropy_model}
\end{figure}


\lnote{
    Suggestions on the implementation.
}

